An Algorithm for Local Transverse Feedback Linearization

Given a multi-input, nonlinear, time-invariant, control-affine system and a controlled invariant, closed, embedded submanifold $\mathsf{N}$, the local transverse feedback linearization (TFL) problem seeks a coordinate and feedback transformation such that, in transformed coordinates, the dynamics governing the system's transverse evolution with respect to $\mathsf{N}$ are linear, time-invariant and controllable. The transformed system is said to be in the TFL normal form. Checkable necessary and sufficient conditions for this problem to be solvable are known, but, unfortunately, the literature does not present a prescription that constructs the required transformation for multi-input systems. In this article we present an algorithm that produces a virtual output of suitable vector relative degree that, using input-output feedback linearization, puts the system into TFL normal form. The procedure is based on dual conditions for TFL and is fundamentally different from existing methods, such as the GS and Blended algorithms, because of the "desired" zero dynamics manifold $\mathsf{N}$. The proposed algorithm is the first to take into consideration the desired zero dynamics manifold.

==> MIMOTFL-Theory-DerivedFlag.tex <==
\subsection{On the Derived Flag}
\label{sec:tech:derivedflag}
First recall the classic \(\CInfty(\Manifold{M})\)-submodules, found as \(\mathscr{M}^l\) in~\cite{Marino1986},
%
\begin{equation}
  \label{eqn:G}
  \Module{G}^k
    \defineas
      \SpanInline{\CInfty(\Manifold{M})}{
        \Ad_f^j g_i \colon 1 \leq i \leq m, 0 \leq j \leq k
      }
      \quad k \geq 0,
\end{equation}
%
as well as the submodules, which can be seen as a variant of \(\mathscr{G}^j\) in~\cite{Marino1986},
%
\begin{equation}
  \label{eqn:S}
  \begin{aligned}
    \Module{S}^0 &\defineas \Module{G}^0,\\
    \Module{S}^k &\defineas
      \Span{\CInfty(\Manifold{M})}{
        \Module{S}^{k-1},
        \left[ \Module{S}^{k-1}, \Module{S}^{k-1} \right],
        \Module{G}^k
      }
      \quad k \geq 1.
  \end{aligned}
\end{equation}
%
These submodules (equivalently their associated distributions) were defined in our previous work~\cite{DSouza2021} in the single input case.
Although \(\Module{G}^k\) and \(\Module{S}^k\) may not be equal, their involutive closures are.
%
\begin{lemma}
  \label{lem:invG}
  For all \(k \geq 0,\) \(\Inv(\Module{G}^k) = \Inv(\Module{S}^k).\)
\end{lemma}
\begin{proof}
  \emph{(\(\subseteq\)):}
  By~\eqref{eqn:S} \(\Module{G}^k \subseteq \Module{S}^k\) and so, by the definition of the involutive closure, we have \(\Inv(\Module{G}^k) \subseteq \Inv(\Module{S}^k).\)

  \emph{(\(\supseteq\)):}
  To show the reverse containment first observe that by definition~\eqref{eqn:S} we have that \(\Inv(\Module{S}^0) = \Inv(\Module{G}^0).\)
  Suppose, by way of induction, that for some \(k\geq 0,\)
  \begin{equation}
    \label{lem:invG:induction}
    \Inv(\Module{S}^k) \subseteq \Inv(\Module{G}^k).
  \end{equation}
  Then by definition~\eqref{eqn:S}{\blue
  \begin{align*}
    \blue
    \Inv(\Module{S}^{k+1})
      &=
        \Inv\left(
          \Span{\CInfty(\Manifold{M})}{
            \Module{S}^{k},
            \left[ \Module{S}^{k}, \Module{S}^{k} \right],
            \Module{G}^{k+1}
          }
        \right),\\
      % &\subseteq
      %   \Inv\left(
      %     \Span{\CInfty(\Manifold{M})}{
      %       \Inv(\Module{S}^{k}),
      %       \left[ \Module{S}^{k}, \Module{S}^{k} \right],
      %       \Module{G}^{k+1}
      %     }
      %   \right),\\
      &\subseteq
        \Inv\left(
          \Span{\CInfty(\Manifold{M})}{
            \Inv(\Module{S}^{k}),
            \Module{G}^{k+1}
          }
        \right).
  \end{align*}
  Now} invoke the inductive hypothesis~\eqref{lem:invG:induction} to get
  \[
    \Inv(\Module{S}^{k+1})
      \subseteq
        \Inv\left(
          \Span{\CInfty(\Manifold{M})}{
            \Inv(\Module{G}^{k}),
            \Module{G}^{k+1}
          }
        \right).
  \]
  From~\eqref{eqn:G} observe that \(\Inv(\Module{G}^k)\subseteq \Inv(\Module{G}^{k+1}).\)
  We can apply this and the fact that \(\Module{G}^{k+1} \subseteq \Inv(\Module{G}^{k+1})\) to conclude{\blue
  \begin{align*}
    \Inv(\Module{S}^{k+1})
      &\subseteq
        \Inv\left(
          \Span{\CInfty(\Manifold{M})}{
            \Inv(\Module{G}^{k+1}),
            \Module{G}^{k+1}
          }
        \right)\\
      % &\subseteq
      %   \Inv\left(
      %     \Inv(\Module{G}^{k+1})
      %   \right)\\
      &=
        \Inv(\Module{G}^{k+1}),
  \end{align*}
  and the induction is complete.}
\end{proof}
%
The newly introduced submodule \(\Module{S}^k\) was shown in~\cite{DSouza2021} to precisely characterize, in the single-input case, the vector fields that are annihilated by the ideal \(\Ideal{I}^{(k+1)}\) and its derived flag.
The proof remains the same in the multi-input case except in the base case of the induction used therein.
%
\begin{lemma}[{\cite[Lemma 4.6]{DSouza2021}}]
  \label{lemma46}
  On an open set \(\OpenSet{U} \subseteq \Manifold{M}\) containing \(p_0\) we have
  \[
    \Ideal{I}^{(k)}
      ={\blue
        \Ann(
          \Module{D}^{(0)}
          +
          \Module{S}^{k - 1}
        )},
    \qquad
    k\geq 1.
  \]
\end{lemma}
%
The next result follows directly from Lemma~\ref{lemma46}.
%
\begin{corollary}[{\cite[Corollary 4.7]{DSouza2021}}]
  \label{cor:distofaugmented}
  On an open set \(\OpenSet{U} \subseteq \Manifold{M}\) containing \(p_0\)
  \[
    \GenerateInline{\Ideal{I}^{(k)}, \D t}
      ={\blue
        \Ann(
          \Module{U}
          +
          \Module{S}^{k - 1}
        )},
    \qquad
    k \geq 1.
  \]
\end{corollary}
%
Given these results, we can show that the differential ideal \(\langle \Ideal{I}^{(k)}, \D t\rangle^{(\infty)}\) is contained in the annihilator of the involutive closure of the control distributions \(\Module{G}^{k-1}.\)
%
\begin{proposition}
  \label{prop:distofclosure}
  On an open set \(\OpenSet{U} \subseteq \Manifold{M}\) containing \(p_0\)
  \[
    \GenerateInline{ \Ideal{I}^{(k)}, \D t}^{(\infty)}
      \subseteq{\blue
        \Ann(
          \Module{U}
          +
          \Inv(\Module{G}^{k-1})
        )},
    \qquad
    k \geq 1.
  \]
\end{proposition}
\begin{proof}
  In an open set \(\OpenSet{U}\) the differential ideal \(\langle \Ideal{I}^{(k)}, \D t \rangle^{(\infty)}\) annihilates a submodule \(\Module{F} \subseteq \SectionsOf{\TangentSpaceOf{\OpenSet{U}}}\) that is closed under the Lie bracket.
  Since \(\langle \Ideal{I}^{(k)}, \D t \rangle^{(\infty)} \subseteq \langle \Ideal{I}^{(k)}, \D t\rangle\) it follows by Corollary~\ref{cor:distofaugmented}
  \[
    \Module{F}
      \supseteq
        \Module{U}
        +
        \Module{S}^{k-1}.
  \]
  Taking the involutive closure of both sides of the above relation find
  \[
    \Module{F}
      \supseteq
        \Module{U}
        +
        \Inv(\Module{S}^{k-1}),
  \]
  where we've used the fact that \(\Module{S}^{k-1}\) is a module consisting of vector fields only in \(\derivation{x^i}\) and, as such, all vector fields in \(\Module{S}^{k-1}\) commute with vector fields in \(\Module{U}.\)
  Using Lemma~\ref{lem:invG} conclude
  \[
    \Module{F}
      \supseteq
        \Module{U}
        +
        \Inv(\Module{G}^{k-1}).
  \]  
\end{proof}
%
The results of this section show which distributions are annihilated by a given ideal.
They connect Isidori's~\cite[Lemma 4.2.2]{Isidori1995}, that an output yielding a certain vector relative degree annihilates certain distributions (but not others), to the dual context where we search for exact differentials living in certain ideals (but not others).


==> MIMOTFL-Theory-RelativeDegree.tex <==
\subsection{On Uniform Vector Relative Degree}
\label{sec:tech:relativedegree}
Regular zero dynamics manifolds are locally the zero dynamics of an output yielding a vector relative degree.
There are already well-known conditions for an output \(h: \Manifold{M} \to \Real^m \) to yield a vector relative degree at a point \(x_0.\)
They are explicitly discussed on~\cite[pg. 220]{Isidori1995}.
In this section, we explore a dual variant of this definition only in the uniform vector relative degree case --- when \(\kappa_1 = \cdots = \kappa_m.\)
Before proving the key technical result of this Section~\ref{sec:tech:relativedegree}, we demonstrate that a scalar function of the state whose differential is in the derived flag must have a Lie derivative along the vector field \(f\) that resides in the preceding ideal of the flag.
%
\begin{proposition}
  \label{prop:LieH}
  Let \(h \in \CInfty(\Manifold{M})\) be a smooth function of the state.
  If there exists an integer \(k \in \Naturals\) so that
  \(
    \D h \in \langle \Ideal{I}^{(k)}, \D t \rangle,
  \)
  then
  \(
    \Lie_{{f}} \D h \in \langle \Ideal{I}^{(k-1)}, \D t \rangle,
  \)
  and \(\Lie_f h\) is a smooth function of the state.
\end{proposition}
\ifthenelse{\boolean{IsArxiv}}{%
\begin{proof}
  Since \(\D h \in \langle \Ideal{I}^{(k)}, \D t \rangle\) we can write
  \[
    \omega = \D h - b\, \D t,
  \]
  for some \(\omega \in \Ideal{I}^{(k)}\) and \(b \in \CInfty(\Manifold{M}).\)
  Feed in the vector field \(Y\) defined in~\eqref{eqn:vfieldsystem} to find
  \[
    \omega(Y) = \D h(Y) - b\, \D t(Y) = \D h(Y) - b.
  \]
  Since \(Y\in \Module{D}^{(0)}\) and \(\omega \in \Ideal{I}^{(k)}\) \(\subseteq\) \(\Ideal{I}^{(0)}\) \(=\) \(\Ann(\Module{D}^{(0)})\) it follows that
  \begin{equation}
    \label{eqn:lieh:1}
    \D h(Y) = b.
  \end{equation}
  Examine the left-hand side of~\eqref{eqn:lieh:1} by applying \(Y,\) from~\eqref{eqn:vfieldsystem},
  \begin{align*}
    \D h(Y)
      &=
        \D h\left(
          \Derivation{t}
          +
          {f}
          +
          \sum_{j = 1}^m {g}_j u^j
        \right)\\
      &=
        \D h\left(\Derivation{t}\right)
        +
        \D h({f})
        +
        \sum_{j = 1}^m u^j \D h({g}_j).
  \end{align*}
  Since \(\D h \in \langle \Ideal{I}^{(1)}, \D t \rangle\) we have by Corollary~\ref{cor:distofaugmented} that \(\D h \in \Ann(\Module{G}^0).\)
  It follows that
  \[
    \D h(Y) 
      =
        \D h\left(\Derivation{t}\right)
        +
        \D h({f}).
  \]
  Now fix \(p \in \Manifold{M}.\)
  Since \(h\) is a smooth function of the state, i.e. \(h = h \circ \iota \circ \pi,\) find that
  \begin{align*}
    \D h_p (Y_p)
      &=
        \D (h \circ \iota \circ \pi)_p \left(
          \left.\Derivation{t}\right|_p
        \right)
        +
        \D h_p\left(\left.{f}\right|_p\right)\\
      &=
        \D (h \circ \iota)_p \left((\pi)_*
          \left.\Derivation{t}\right|_p
        \right)
        +
        \D h_p\left(\left.{f}\right|_p\right)\\
      &=
        \D h_p\left(\left.{f}\right|_p\right)\\
      &=
        \Lie_{{f}} h(p).
  \end{align*}
  Combine this with~\eqref{eqn:lieh:1} to find \(\Lie_{{f}} h = b.\)
  As a result we may write
  \[
    \omega = \D h - \Lie_{{f}} h\, \D t \in \Ideal{I}^{(k)}.
  \]
  Now compute the exterior derivative to find
  \[
    \D \omega = \D t \wedge \D \Lie_{{f}} h.
  \]
  Evaluating this two-form with \(Y\) gives,
  \begin{align*}
    \D \omega(Y, \cdot)
      &=
        \D t(Y)\,
          \D \Lie_{{f}} h
          \left(
            \vphantom{\Lie_{{f}} h}
            \cdot
          \right)
        -
        (\D \Lie_{{f}} h)(Y)\,
          \D t(\cdot)\\
      &=
        (\D \Lie_{{f}} h)
        \left(
          \vphantom{\Lie_{{f}} h}
          \cdot
        \right)
        -
        \Lie_Y \Lie_{{f}} h\, \D t(\cdot).
  \end{align*}
  Since \(\omega \in \Ideal{I}^{(k)}\) we must have, by the definition of the derived flag, \(\D \omega \in \Ideal{I}^{(k-1)}.\)
  Moreover, \(Y \in \Module{D}^{(0)}\) and \(\Ann(\Module{D}^{(0)})\subseteq \Ideal{I}^{(k-1)}.\)
  Combine these to conclude \(\D \omega(Y, \cdot) \in \Ideal{I}^{(k-1)}.\)
  It immediately follows that
  \[
    \D \Lie_{{f}} h \in \Generate{\Ideal{I}^{(k-1)}, \D t}.
  \]
  Since \(\Lie_{{f}} \D h = \D \Lie_{{f}} h\) the Proposition is proven.
\end{proof}%
}{%
\begin{proof}
  The proof can be found in~\cite{DSouza2021b}, the preprint version of this article.
  For brevity, it is not included in this article.
\end{proof}%
}%
%
Note that Proposition~\ref{prop:LieH} does not assume relative degree and is true for any exact form in \(\langle \Ideal{I}^{(k)}, \D t\rangle,\) for \(k \in \Naturals,\) that is solely state dependent.
The next proposition presents an explicit condition for a family of outputs to have \emph{uniform} vector relative degree.
It can be viewed as a partial dual of the definition of relative degree provided on~\cite[pg. 220]{Isidori1995}.
%
\begin{proposition}
  \label{prop:relativedegree}
  Suppose \(h^1,\) \(\ldots,\) \(h^\ell \in \CInfty(\Manifold{M}),\) \(\ell \leq m,\) are smooth functions of the state with linearly independent differentials at \(p_0.\)
  The system~\eqref{eqn:systemOnM} with output \((h^1,\) \(\ldots,\) \(h^\ell)\) yields a vector relative degree \((\kappa_1,\) \(\ldots,\) \(\kappa_1)\) at \(p_0\) if, and only if, there exists an open set \(\OpenSet{U} \subseteq \Manifold{M}\) containing \(p_0\) where,
  \begin{equation}
    \label{prop:relativedegree:a}
    \GenerateInline{\D h^1, \ldots, \D h^\ell}
    \subseteq
    \GenerateInline{\Ideal{I}^{(\kappa_1 - 1)}, \D t}^{(\infty)}
  \end{equation}
  and, at \(p_0,\)
  \begin{equation}
    \label{prop:relativedegree:b}
    \SpanInline{\Real}{
      \D h^1_{p_0}, \ldots, \D h^\ell_{p_0}
    }
    \cap
    \SpanInline{\Real}{
      \Codist{I}^{(\kappa_1)}_{p_0},
      \D t_{p_0}
    }
    =
    \{
      0
    \}.
  \end{equation}
\end{proposition}
%
Proposition~\ref{prop:relativedegree} only addresses those outputs with uniform relative degree because the non-uniform case involves ensuring the scalar outputs and their Lie derivatives form an adapted basis that generates the ideals in the derived flag.
This result is useful for finding and verifying outputs that yield uniform vector relative degree.
%
\ifthenelse{\boolean{IsArxiv}}{%
\begin{proof}[Proof of Proposition~\ref{prop:relativedegree}]
  Let \(h^1,\) \(\ldots,\) \(h^\ell \in \CInfty(\Manifold{M}),\) \(\ell \leq m,\) be smooth functions of the state with linearly independent differentials at \(p_0 \in \Manifold{M}.\)
  First we suppose the conditions~\eqref{prop:relativedegree:a} and~\eqref{prop:relativedegree:b} hold and prove the system~\eqref{eqn:systemOnM} with output \((h^1,\) \(\ldots,\) \(h^\ell)\) yields a vector relative degree \((\kappa_1,\) \(\ldots,\) \(\kappa_1)\) at \(p_0.\)
  For each \(i \in \{1, \ldots, \ell\}\) apply Proposition~\ref{prop:distofclosure} and use the fact that
  \(
    \D h^i \in \langle \Ideal{I}^{(\kappa_1-1)}, \D t \rangle^{(\infty)}
  \)
  to arrive at
  \[
    \D h^i \in \Ann(\Inv(\Module{G}^{\kappa_1 - 2})).
  \]
  This implies
  \[
    \Lie_{\Ad_f^j g_l} h^i
      = \D h^i ( \Ad_{{f}}^{j} g_l )
      = 0,
    \quad 0 \leq j \leq \kappa_1 - 2, 1 \leq l \leq m, 1 \leq i \leq \ell. 
  \]

  We now show that the associated \(\ell \times m\) decoupling matrix has rank \(\ell\) at \(p_0.\)
  In pursuit of contradiction, suppose there exists constants \(c_i \in \Real\) so that
  \[
    \sum_{i = 1}^\ell
      c_i
      \left.
        \Lie_{\begin{bsmallmatrix} {g}_1 & \cdots & {g}_m\end{bsmallmatrix}}
        \Lie_{{f}}^{\kappa_1 - 1}
        h^i
      \right|_{p_0}
      =
        0.
  \]
  Define the smooth function
  \[
    h \defineas \sum_{i = 1}^\ell c_i h^i
    \in \CInfty(\Manifold{M}).
  \]
  Since
  \(
    \D h^i \in \langle \Ideal{I}^{(\kappa_1 - 1)}, \D t\rangle^{(\infty)}
  \)
  and \(c_i\in \Real,\) we have
  \(
    \D h \in \langle \Ideal{I}^{(\kappa_1 - 1)}, \D t\rangle^{(\infty)}.
  \)
  For any fixed \(1 \leq l \leq m,\) consider
  \(
    \D h( \Ad_{{f}}^{\kappa_1 - 1} g_l).
  \)
  By \cite[Lemma 4.1.2]{Isidori1995}\footnote{We consider when \(s = 0,\) \(k = 0\) and \(r = \kappa_1 - 1.\)},
  \[
    \D h\left( \Ad_{{f}}^{\kappa_1 - 1} {g_l}\right)
      =
        \sum_{i = 0}^{\kappa_1 - 1}
          (-1)^i
          \begin{pmatrix}
            \kappa_1 - 1 \\ i
          \end{pmatrix}
          \Lie_{{f}}^{\kappa_1 - 1 - i}
          \Lie_{g_l} \Lie_{f}^{i} h.
  \]
  By Proposition~\ref{prop:LieH}, \(\Lie_{{f}}^i \D h \in \Ann(\Module{G}^0)\) for all \(0 \leq i \leq \kappa_1 - 2\) and, as a result,
  \[
    \D h\left( \Ad_f^{\kappa_1 - 1} g_l\right)
      =
        (-1)^{\kappa_1 - 1}
        \Lie_{g_l} \Lie_f^{\kappa_1 - 1} h.
  \]
  Evaluating at \(p_0\)
  \[
    \D h_{p_0}\left( \Ad_f^{\kappa_1 - 1} g_l(p_0) \right)
      =
        (-1)^{\kappa_1 - 1}
        \Lie_{g_l} \Lie_f^{\kappa_1 - 1} h(p_0)
      =
        0.
  \]
  Since \(1 \leq l \leq m\) was arbitrary, \(\D h_{p_0} \in \Ann( \Dist{G}^{\kappa_1 - 1} ).\)
  But then, by Corollary~\ref{cor:distofaugmented} and the fact that \(\D h\) is exact,
  \[
    \D h_{p_0} \in \Span{\Real}{\Codist{I}^{(\kappa_1)}_{p_0}, \D t_{p_0}}
  \]
  which, in tandem with~\eqref{prop:relativedegree:b}, implies
  \[
    \D h_{p_0} = 0, \quad k \in \Real.
  \]
  This contradicts the preliminary assumption of Proposition~\ref{prop:relativedegree} that the differentials \(\D h^i\) are linearly independent at \(p_0 \in \OpenSet{U}.\)
  Therefore the decoupling matrix has maximal rank and so it follows that the outputs yield a well-defined vector relative degree.

  Now suppose the output \((h^1,\) \(\ldots,\) \(h^\ell)\) yields a vector relative degree of \((\kappa_1,\) \(\ldots\) \(\kappa_1)\) at \(p_0.\)
  Fix \(1 \leq i \leq m\) and \(1 \leq j \leq \ell.\)
  By~\cite[Lemma 4.1.2]{Isidori1995} and the definition of relative degree we have
  \[
  \begin{aligned}
    \D h^j\left(\Ad_f^{k} g_i\right)
      &= \Lie_{\Ad_f^{k} g_i} h^j,\\
      &= 0,
      \quad
      0 \leq k \leq \kappa_1 - 2.
  \end{aligned}
  \]
  We may conclude \(\D h^j \in \Ann(\Module{G}^k)\) for all \(0 \leq k \leq \kappa_1 - 2.\)
  Since \(\D h^j\) is exact, it is easy to see that for any two vector fields \(X, Y \in \Module{G}^k\) we have 
  \[
    \Lie_{[X,Y]} h^j
      = \Lie_X\left(\Lie_Y h^j\right) - \Lie_Y\left(\Lie_X h^j\right) = 0,
  \]
  So \(\D h^j\) annihilates any finite order Lie brackets of vector fields in \(\Module{G}^k.\)
  We now show by induction that \(\D h^j\) annihilates any finite order Lie brackets of vector fields in \(\Module{S}^k.\)
  First see that \(\Module{S}^0 = \Module{G}^0\) so we have \(\D h^j \in \Module{S}^0.\)
  Therefore \(\D h^j\) also annihilates any finite order Lie brackets of vector fields in \(\Module{S}^0.\)
  By way of induction suppose \(\D h^j \in \Module{S}^{k}\) and that it annihilates finite order Lie brackets of vector fields in \(\Module{S}^k.\)
  Then, by~\eqref{eqn:S}, the fact that \(\D h^j \in \Ann(\Module{G}^k)\) and \(\D h^j \in \Ann(\Module{S}^k)\) and the fact that it annihilates finite order of Lie brackets for \(\Module{S}^{k-1}\) conclude that \(\D h^j \in \Ann(\Module{S}^k).\)
  This argument holds until \(k = \kappa_1 - 2.\)
  As such we have
  \[
    \D h^j \in \Ann(\Module{S}^k), \quad 0 \leq k \leq \kappa_1 - 2.
  \]
  Since \(\D h^j\) is independent of \(u,\) we have that
  \(
    \D h^j
      \in
        \Ann(
          \Module{U}
        ),
  \)
  so by Corollary~\ref{cor:distofaugmented}
  \[
    \D h^j \in \Generate{ \Ideal{I}^{(\kappa - 1)}, \D t}.
  \]
  Since \(\D h^j\) is exact, it is closed and so 
  \[
    \D h^j \in \Generate{ \Ideal{I}^{(\kappa - 1)}, \D t}^{(\infty)}
  \]
  Since \(j \in \{1,\) \(\ldots,\) \(m\}\) was arbitrary, this demonstrates that~\eqref{prop:relativedegree:a} holds.
  We now show that~\eqref{prop:relativedegree:b} holds as well by a contrapositive argument.
  Suppose that~\eqref{prop:relativedegree:b} does not hold. 
  We will show that the output does not yield a vector relative degree.
  Given that the condition~\eqref{prop:relativedegree:b} fails, there must exist a linear combination of the \(\D h^i\) so that
  \[
    \sum_{i=1}^\ell a_i \D h^i_{p_0}
    \in
    \Span{\Real}{\Codist{I}^{(\kappa)}_{p_0}, \D t_{p_0}}.
  \]
  By Corollary~\eqref{cor:distofaugmented} and~\eqref{eqn:S},
  \[
    \sum_{i=1}^\ell a_i \D h^i
    \in
    \Ann\left( \Module{G}^{\kappa - 1} \right)
  \]
  and, in particular,
  \[
    \sum_{i=1}^\ell a_i \D h^i\left( \Ad_f^{\kappa - 1} g_j \right) = 0, \quad 1 \leq j \leq m.
  \]
  on \(\OpenSet{U}.\)
  By~\cite[Lemma 4.1.2]{Isidori1995} and because \(\sum a_i \D h^i \in \Ann(\Module{G}^k)\) for \(0 \leq k \leq \kappa_2 - 2,\)
  \[
    \sum_{i=1}^\ell a_i \Lie_{g_j} \Lie_f^{\kappa - 1} h^i = 0,
    \quad 1 \leq j \leq m.
  \]
  This contradicts the requirement that the decoupling matrix 
  \(
    \Lie_{\begin{bsmallmatrix}g_1 & \cdots & g_m\end{bsmallmatrix}} \Lie_f^{\kappa - 1} h
  \)
  has maximal row rank and so the outputs do not yield a vector relative degree.
\end{proof}%
}{%
\begin{proof}[Proof of Proposition~\ref{prop:relativedegree}]
  The proof can be found in~\cite{DSouza2021b}, the preprint version of this article.
  For brevity, it is not included in this article.
\end{proof}%
}%
%

